Ridge Regression and Provable Deterministic Ridge Leverage Score Sampling

Ridge leverage scores provide a balance between low-rank approximation and regularization, and are ubiquitous in randomized linear algebra and machine learning. Deterministic algorithms are also of interest in the moderately big data regime, because deterministic algorithms provide interpretability to the practitioner by having no failure probability and always returning the same results. We provide provable guarantees for deterministic column sampling using ridge leverage scores. The matrix sketch returned by our algorithm is a column subset of the original matrix, yielding additional interpretability. Like the randomized counterparts, the deterministic algorithm provides (1 + {\epsilon}) error column subset selection, (1 + {\epsilon}) error projection-cost preservation, and an additive-multiplicative spectral bound. We also show that under the assumption of power-law decay of ridge leverage scores, this deterministic algorithm is provably as accurate as randomized algorithms. Lastly, ridge regression is frequently used to regularize ill-posed linear least-squares problems. While ridge regression provides shrinkage for the regression coefficients, many of the coefficients remain small but non-zero. Performing ridge regression with the matrix sketch returned by our algorithm and a particular regularization parameter forces coefficients to zero and has a provable (1 + {\epsilon}) bound on the statistical risk. As such, it is an interesting alternative to elastic net regularization.

==> conclusion.tex <==
We extend deterministic feature selection from rank-$k$ subspace leverage scores to ridge leverage scores.  Ridge leverage scores provide a natural and stable alternative to rank-$k$ subspace leverage scores for decreasing the importance of small principle components \citep{cohen_input_2017}.  Deterministic algorithms provide interpretability over their randomized counterparts.

We provide guarantees on the performance of our deterministic algorithm with respect to $(1+\epsilon)$ error column subset selection, $(1+\epsilon)$ error projection-cost preservation, and an additive-multiplicative spectral bound.  These guarantees improve upon the available guarantees for deterministic feature selection with rank-$k$ subspace leverage scores, and are comparable to randomized ridge leverage score algorithms under the assumption of power-law decay.  We also show a $(1+\epsilon)$ error guarantee on the statistical risk for ridge regression with a particular regularization constant and using the column subset from our deterministic algorithm.  A similar ridge regression risk bound holds for randomized ridge leverage sampling.    Lastly, we include a biological application to show that ridge leverage score power-law decay exists in the wild.


